The Cosmology Large Angular Scale Surveyor (CLASS): 38 GHz detector array of bolometric polarimeters

The Cosmology Large Angular Scale Surveyor (CLASS) experiment aims to map the polarization of the Cosmic Microwave Background (CMB) at angular scales larger than a few degrees. Operating from Cerro Toco in the Atacama Desert of Chile, it will observe over 65% of the sky at 38, 93, 148, and 217 GHz. In this paper we discuss the design, construction, and characterization of the CLASS 38 GHz detector focal plane, the first ever Q-band bolometric polarimeter array.

==> questions.tex <==

CLASS observes 65\% of all sky? or extragalactic sky?

E and B modes , rank 2-tensor fields

Galactic sysncrotorn dominates at below? 70 GHz

Frequencies 40, 90, 150,? ok?

clip mounting scheme, showen on picture? diagram?

spring clip tungsten?

pure silicon crystal dielectric?

shunt, nyquist?

lenght of traces 1-6 inch? calculate inductance?

double chack num of opt-dark-squid= 72-4-12

tech etch wedsite, info

tek data website info

MDM info

tek data, inter wound? woven?

what tolerances is the plate machining?

do we want a diagram of circuit layout? 

do we want diagram of FP?

do we want diagram of clip?

picture caption?

